Convergence results for a coarsening model using global linearization

We study a coarsening model describing the dynamics of interfaces in the one-dimensional Allen-Cahn equation. Given a partition of the real line into intervals of length greater than one, the model consists in constantly eliminating the shortest interval of the partition by merging it with its two neighbors. We show that the mean-field equation for the time-dependent distribution of interval lengths can be explicitly solved using a global linearization transformation. This allows us to derive rigorous results on the long-time asymptotics of the solutions. If the average length of the intervals is finite, we prove that all distributions approach a uniquely determined self-similar solution. We also obtain global stability results for the family of self-similar profiles which correspond to distributions with infinite expectation.

==> fig1.tex <==
% height 5.5 cm
% width 11.0 cm 
\smash{\hbox{
\point  1.00    9.90    {$\theta=0.5$}
\point  8.50    9.90    {$\theta=1.0$}
\point  1.00    4.20    {$\theta=2.0$}
\point  8.50    4.20    {$\theta=3.5$}
}}



==> fig2.tex <==
% height 5.5 cm
% width 11.0 cm 
\smash{\hbox{
\point  0.70    0.70    {${\rm a}$}
\point  8.70    0.70    {${\rm b}$}
\point  2.50    3.30    {$\wh w_1^*$}
\point  11.00   3.70    {$1{-}\e^{-\wh w_1^*}$}
}}


